Some examples of quantum graphs

We summarize different approaches to the theory of quantum graphs and provide several ways to construct concrete examples. First, we classify all undirected quantum graphs on the quantum space $M_2$. Secondly, we apply the theory of 2-cocycle deformations to Cayley graphs of abelian groups. This defines a twisting procedure that produces a quantum graph, which is quantum isomorphic to the original one. For instance, we define the anticommutative hypercube graphs. Thirdly, we construct an example of a quantum graph, which is not quantum isomorphic to any classical graph.

==> graphmor.tex <==
\def\Gsing{\Graph{
\draw (1,0.5) node{} -- (1,0);
}}

\def\Gupsing{\Graph{
\draw (1,0.5) node{} -- (1,1);
}}
%
\def\Gpair{\Graph{
\draw (1,0) -- (1,0.3) -- (1.5,0.5) node {} -- (2,0.3) -- (2,0);
}}
%
\def\Guppair{\Graph{
\draw (1,1) -- (1,0.7) -- (1.5,0.5) node {} -- (2,0.7) -- (2,1);
}}

\def\Gconnecter{\Graph{
\draw (1,0) -- (1,0.3) -- (1.5,0.5) -- (2,0.3) -- (2,0);
\draw (1,1) -- (1,0.7) -- (1.5,0.5) node {} -- (2,0.7) -- (2,1);
}}
%
%\def\GEconnecter{\Graph{
%\GE 0.7/0.5:1/1.5,2/1.5;
%\GE 0.3/0.5:1/1.5,2/1.5;
%\GS 0.7/1:1/,2/;
%\GS 0.3/0:1/,2/;
%\GV 0.5:1.5;
%\GV 0.3:1,2;
%\GV 0.7:1,2;
%}}
%
\def\Gfork{\Graph{
%\GS 0.3/0.5:1/1.5,2/1.5;
%\GS 0.5/1:1.5/;
%\GS 0.3/0:1/,2/;
%\GV 0.5:1.5;
\draw (1.5,0.5) -- (2,0.3) -- (2,0);
\draw (1.5,1) -- (1.5,0.5) node {} -- (1,0.3) -- (1,0);
}}
%
\def\Gmerge{\Graph{
%\GS 0.7/0.5:1/1.5,2/1.5;
%\GS 0.7/1:1/,2/;
%\GS 0.5/0:1.5/;
%\GV 0.5:1.5;
\draw (1.5,0.5) -- (2,0.7) -- (2,1);
\draw (1.5,0) -- (1.5,0.5) node{} -- (1,0.7) -- (1,1);
}}
%
%\def\Gfour{\Graph{
%\GS 0.3/0.5:1/2.5,2/2.5,3/2.5,4/2.5;
%\GS 0.3/0:1/,2/,3/,4/;
%\GV 0.5:2.5;
%}}
%
%\def\Gcross{\Graph{
%\GS 0/1:1/2,2/1;
%\GV 0.75:1.25,1.75;
%}}
%
%\def\Ggrpth{\Graph{
%\GV 0.5:2;
%\GV 0.8:1.4;
%\GS 0.5/1:2/2,2/3;
%\GS 0.5/0:2/1,2/2;
%\GS 0.8/1:1.4/1;
%\GS 0.2/0:2.6/3;
%\GSa (1.4,0.8) (-0.6,0.3) (0.25,0.25)
%}}
%
%\def\GA{\Graph{
%\GE 0.25/0.75:1/;
%\GS 0/0.25:1/;
%\GS 0.75/1:1/;
%\GV 0.25:1;
%\GV 0.75:1;
%}}
%
%\def\GAA{\Graph{
%\GE 0.25/0.75:1.15/;
%\GE 0.25/0.75:0.85/;
%\GS 0/0.25:1/;
%\GS 0.75/1:1/;
%\GV 0.25:1;
%\GV 0.75:1;
%}}


\def\Graph#1{%
\ifmmode
\mathchoice{
\,\GraphA{0.25em}{1em}{1em}{#1}\,%
}{
\,\GraphA{0.25em}{0.7em}{1em}{#1}\,%
}{
\,\GraphA{0.175em}{0.55em}{0.7em}{#1}\,%
}{
\,\GraphA{0.125em}{0.4em}{0.5em}{#1}\,%
}\else%
\thinspace\GraphA{0.25em}{0.7em}{1em}{#1}\thinspace%
\fi%
}

\def\GraphA#1#2#3#4{%
\expandafter\tikzpicture\Gparam
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
#4
\endtikzpicture
}

\def\Gblack{\def\Gparam{[every node/.style={circle,draw,fill=black,inner sep=1pt},]}}
\def\Gwhite{\def\Gparam{[every node/.style={circle,draw,fill=white,inner sep=1pt},]}}
\def\Gsquare{\def\Gparam{[every node/.style={draw,fill=white,inner sep=1pt},]}}
\def\Gbox{\def\Gparam{[every node/.style={draw,inner sep=1pt},]}}

\Gblack


==> partmac.tex <==
%%Macro package for typeseting set partitions
%%Daniel Gromada 2019--2020
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%First, also as an example, we define shortcuts for some short partitions using word representation.

%%%Partitions with lower points only

%%k=1

\def\La{\LPartition{0.6:1}{}}

%%k=2

\def\Laa{\LPartition{}{0.6:1,2}}
\def\Lab{\LPartition{0.6:1,2}{}}

%k=3

\def\Laaa{\LPartition{}{0.6:1,2,3}}
\def\Laab{\LPartition{0.6:3}{0.6:1,2}}
\def\Laba{\LPartition{0.4:2}{0.8:1,3}}
\def\Labb{\LPartition{0.6:1}{0.6:2,3}}
\def\Labc{\LPartition{0.6:1,2,3}{}}

%k=4


\def\Laaaa{\LPartition{}{0.6:1,2,3,4}}
\def\Laaab{\LPartition{0.6:4}{0.6:1,2,3}}
\def\Laaba{\LPartition{0.4:3}{0.8:1,2,4}}
\def\Labaa{\LPartition{0.4:2}{0.8:1,3,4}}
\def\Labbb{\LPartition{0.6:1}{0.6:2,3,4}}
\def\Laabb{\LPartition{}{0.6:1,2;0.6:3,4}}
\def\Labba{\LPartition{}{0.8:1,4;0.4:2,3}}
\def\Labab{\LPartition{}{0.8:2,4;0.4:1,3}}
\def\Laabc{\LPartition{0.6:3,4}{0.6:1,2}}
\def\Labac{\LPartition{0.4:2,4}{0.8:1,3}}
\def\Labca{\LPartition{0.4:2,3}{0.8:1,4}}
\def\Labbc{\LPartition{0.6:1,4}{0.6:2,3}}
\def\Labcb{\LPartition{0.4:1,3}{0.8:2,4}}
\def\Labcc{\LPartition{0.6:1,2}{0.6:3,4}}
\def\Labcd{\LPartition{0.6:1,2,3,4}{}}

%%%Partitions with upper points only

%%k=1

\def\Ua{\UPartition{0.4:1}{}}

%%k=2

\def\Uaa{\UPartition{}{0.4:1,2}}
\def\Uab{\UPartition{0.4:1,2}{}}

%k=3

\def\Uaaa{\UPartition{}{0.5:1,2,3}}
\def\Uaab{\UPartition{0.4:3}{0.4:1,2}}
\def\Uaba{\UPartition{0.6:2}{0.2:1,3}}
\def\Uabb{\UPartition{0.4:1}{0.4:2,3}}
\def\Uabc{\UPartition{0.4:1,2,3}{}}

%k=4

\def\Uaaaa{\UPartition{}{0.4:1,2,3,4}}
\def\Uaaab{\UPartition{0.4:4}{0.4:1,2,3}}
\def\Uaaba{\UPartition{0.6:3}{0.2:1,2,4}}
\def\Uabaa{\UPartition{0.6:2}{0.2:1,3,4}}
\def\Uabbb{\UPartition{0.4:1}{0.4:2,3,4}}
\def\Uaabb{\UPartition{}{0.4:1,2;0.4:3,4}}
\def\Uabba{\UPartition{}{0.2:1,4;0.6:2,3}}
\def\Uabab{\UPartition{}{0.2:2,4;0.6:1,3}}
\def\Uaabc{\UPartition{0.4:3,4}{0.4:1,2}}
\def\Uabac{\UPartition{0.6:2,4}{0.2:1,3}}
\def\Uabca{\UPartition{0.6:2,3}{0.2:1,4}}
\def\Uabbc{\UPartition{0.4:1,4}{0.4:2,3}}
\def\Uabcb{\UPartition{0.6:1,3}{0.2:2,4}}
\def\Uabcc{\UPartition{0.4:1,2}{0.4:3,4}}
\def\Uabcd{\UPartition{0.4:1,2,3,4}{}}

%%%Partitions with same amount of upper and lower points

%%k=1, l=1

\def\Paa{\Partition{
\Pline (1,0) (1,1)
}}

\def\Pab{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
}}

%k=4

\def\Paaaa{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
\Pline (1.5,0.3) (1.5,0.7)
}}
\def\Paaab{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:2
\Pline (1,0) (1,0.7)
}}
\def\Paaba{\Partition{
\Pblock 1to0.7:1,2
\Psingletons 0to0.3:1
\Pline (2,0) (2,0.7)
}}
\def\Pabaa{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1
\Pline (2,0.3) (2,1)
}}
\def\Pabbb{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:2
\Pline (1,0.3) (1,1)
}}
\def\Paabb{\Partition{
\Pblock 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabba{\Partition{
\Pline (1,0) (1,1)
\Pline (2,0) (2,1)
}}
\def\Pabab{\Partition{
\Pline (1,0) (2, 1)
\Pline (1,1) (2, 0)
}}
\def\Paabc{\Partition{
\Psingletons 0to0.3:1,2
\Pblock 1to0.7:1,2
}}
\def\Pabcc{\Partition{
\Pblock 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}
\def\Pabac{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:1
\Pline (1,0) (2,1)
}}
\def\Pabcb{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:2
\Pline (2,0) (1,1)
}}
\def\Pabca{\Partition{
\Psingletons 0to0.3:1
\Psingletons 1to0.7:1
\Pline (2,0) (2,1)
}}
\def\Pabbc{\Partition{
\Psingletons 0to0.3:2
\Psingletons 1to0.7:2
\Pline (1,0) (1,1)
}}
\def\Pabcd{\Partition{
\Psingletons 0to0.3:1,2
\Psingletons 1to0.7:1,2
}}

%k=6

\def\Pabcabc{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
}}
\def\Pabcabd{\Partition{
\Pline (1,0) (3, 1)
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:3
\Psingletons 1to0.7:1
}}
\def\Pabcadc{\Partition{
\Pline (1,0) (3, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:2
\Psingletons 1to0.8:2
}}
\def\Pabcdbc{\Partition{
\Pline (2,0) (2, 1)
\Pline (3,0) (1, 1)
\Psingletons 0to0.3:1
\Psingletons 1to0.7:3
}}
\def\Pabcade{\Partition{
\Pline (1,0) (3, 1)
\Psingletons 0to0.2:2,3
\Psingletons 1to0.8:1,2
}}
\def\Pabcdec{\Partition{
\Pline (3,0) (1, 1)
\Psingletons 0to0.2:1,2
\Psingletons 1to0.8:2,3
}}
\def\Pabcdbe{\Partition{
\Pline (2,0) (2, 1)
\Psingletons 0to0.3:1,3
\Psingletons 1to0.7:1,3
}}
\def\Pabcdef{\Partition{
\Psingletons 0to0.3:1,2,3
\Psingletons 1to0.7:1,2,3
}}

\def\Paabaab{\Partition{
\Pblock 1to0.75:2,3
\Pblock 0to0.25:1,2
\Pline (1.5,0.25)(2.5,0.75)
\Pline (3,0)(1,1)
}}

%%%Some aliases

%\def\singleton{{\mathord{\uparrow}}}
%\def\upsingleton{{\mathord{\downarrow}}}
\def\singleton{\LPartition{\Ps1:1}{}}
\def\upsingleton{\UPartition{\Ps0:1}{}}
\let\pairpart=\Laa
\let\uppairpart=\Uaa
\let\fourpart=\Laaaa
\let\idpart=\Paa
\let\disconnecterpart=\Pab
\let\connecterpart=\Paaaa
\let\crosspart=\Pabab
\let\positionerpart=\Pabcb
\let\halflibpart=\Pabcabc


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%The macros

\def\textchoice#1#2#3#4#5{\ifmmode\mathchoice{#1}{#2}{#3}{#4}\else #5\fi}
\def\fihere#1\fi{\fi#1}

%definition of the \Partition command
\def\Partition#1{\def\Ptmp{#1}%
\futurelet\nextchar\PartitionB
}

\def\BigPartition#1{\def\Ptmp{#1}%
\futurelet\nextchar\BigPartitionB
}

\def\PartitionD{%
\thinspace\textchoice
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}
{\PartitionA{0.175em}{0.55em}{0.7em}{\Ptmp}}
{\PartitionA{0.125em}{0.4em}{0.5em}{\Ptmp}}
{\PartitionA{0.25em}{0.7em}{1em}{\Ptmp}}%
\thinspace%
}

\def\BigPartitionD{%
\thinspace\textchoice
{\PartitionA{1em}{0.9em}{2.5em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}
{\PartitionA{0.25em}{0.5em}{1em}{\Ptmp}}
{\PartitionA{0.20em}{0.4em}{0.8em}{\Ptmp}}
{\PartitionA{0.75em}{0.7em}{2em}{\Ptmp}}%
\thinspace
}

\newcount\tmpx
\newcount\tmpy
\def\PartitionB{\if[\nextchar\let\next=\PartitionC\else\let\next=\PartitionD\fi\next}
\def\BigPartitionB{\if[\nextchar\let\next=\BigPartitionC\else\let\next=\BigPartitionD\fi\next}
\def\PartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\PartitionD}
\def\BigPartitionC[#1]{\tmpx=0\tmpy=0\expandafter\def\expandafter\Ptmp\expandafter{\Ptmp\Ppointlist#1]}\BigPartitionD}

\def\Ppointlist#1{\advance\tmpx by 1\if#1]\else
	\csname P#1\endcsname(\the\tmpx,\the\tmpy)
	\fihere\Ppointlist\fi}

\def\Pwidth{0.05}

\def\Phook{}

\def\PartitionA#1#2#3#4{%
\pgfpicture
\pgfsetbaseline{#1}
\pgfsetxvec{\pgfpoint{#2}{0em}}
\pgfsetyvec{\pgfpoint{0em}{#3}}
\pgfsetlinewidth{\Pwidth em}
\Phook
#4
\endpgfpicture
}

%\Pline, \Psingletons, \Pblock, \Ptext,...

\def\Pline(#1,#2)#3(#4,#5){
\pgfpathmoveto{\pgfpointxy{#1}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#5}}
\pgfusepath{stroke}
}

\def\Psingletons #1to#2:#3 {\PsingletonsA{#1}{#2}#3,,}
\def\PsingletonsA#1#2#3,{\ifx,#3,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfusepath{stroke}
\fihere\PsingletonsA{#1}{#2}\fi}

\def\Pblock #1to#2:#3 {\PblockA{#1}{#2}#3,,
\pgfusepath{stroke}
}
\def\PblockA#1#2#3,#4,{\ifx,#4,\else
\pgfpathmoveto{\pgfpointxy{#3}{#1}}
\pgfpathlineto{\pgfpointxy{#3}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#2}}
\pgfpathlineto{\pgfpointxy{#4}{#1}}
\fihere\PblockA{#1}{#2}#4,\fi}

\def\Ptext(#1,#2)#3{%
\pgftext[at={\pgfpointxy{#1}{#2}}]{#3}
}

%\LPartition,\Upartition

\def\LPartition#1#2{\Partition{
\LPartitionB#2;;
\LPartitionA#1;;
}}

\def\LPartitionA#1;{\ifx;#1;\else
\Lsingletons #1 
\fihere\LPartitionA\fi}

\def\LPartitionB#1;{\ifx;#1;\else
\Pblock 0to#1 
\fihere\LPartitionB\fi}

\def\UPartition#1#2{\Partition{
\UPartitionB#2;;
\UPartitionA#1;;
}}

\def\UPartitionA#1;{\ifx;#1;\else
\Usingletons #1 
\fihere\UPartitionA\fi}

\def\UPartitionB#1;{\ifx;#1;\else
\Pblock 1to#1 
\fihere\UPartitionB\fi}

\def\Lsingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint0 #1#2 \else\Psingletons 0to#1#2 \fi
}
\def\Usingletons #1#2 {%
	\ifcat\noexpand#1\noexpand\ \Ppoint1 #1#2 \else\Psingletons 1to#1#2 \fi
}

%colors

\def\Pcolw{0.1}

\expandafter\def\csname P/\endcsname{\advance\tmpy by1 \tmpx=0}
\expandafter\def\csname P0\endcsname{}

\def\Pw (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
}

\def\Pb (#1,#2){
	\pgfpathcircle{\pgfpointxy{#1}{#2}}{\Pcolw em}
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
}

\def\Ps#1(#2,#3){
	\pgfsetarrowsend{to}
	\pgfpathmoveto{\pgfpointxy{#2}{#3}}
	\pgfpathlineto{\pgfpointxy{#2}{#1}}
	\pgfusepath{stroke}
	\pgftransformreset
	\pgfsetarrowsend{}
}

\def\Pq (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{white}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\PQ (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	\pgfpathmoveto{\pgfpoint{-\Pcolw em}{-\Pcolw em}}
	\pgfpathlineto{\pgfpoint{-\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{\Pcolw em}}
	\pgfpathlineto{\pgfpoint{\Pcolw em}{-\Pcolw em}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}
	\pgftransformreset
}

\def\Lt (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\Ut (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfusepath{stroke}}
	\pgftransformreset
}
\def\LT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}
\def\UT (#1,#2){
	\pgftransformshift{\pgfpointxy{#1}{#2}}
	{\pgfsetxvec{\pgfpoint{\Pcolw em}{0em}}
	\pgfsetyvec{\pgfpoint{0em}{\Pcolw em}}
	\pgfpathmoveto{\pgfpointxy{-1.4}{0}}
	\pgfpathlineto{\pgfpointxy{0}{-2.5}}
	\pgfpathlineto{\pgfpointxy{1.4}{0}}
	\pgfpathclose
	\pgfsetfillcolor{black}
	\pgfusepath{stroke,fill}}
	\pgftransformreset
}

\def\Ppoint #1 #2:#3 {\PpointA{#1}{#2}#3,,}
\def\PpointA#1#2#3,{\ifx,#3,\else #2(#3,#1)\fihere\PpointA{#1}{#2}\fi}

\def\coldefA #1 #2{\kern0.1ex\vcenter{\hbox{\def\Pcolw{#1}\pgfpicture#2(0,0)\endpgfpicture}}\kern0.1ex}

\def\coldef#1#2{\def#1{{\textchoice
{\coldefA 0.15 #2}{\coldefA 0.15 #2}{\coldefA 0.1 #2}{\coldefA 0.08 #2}{$\coldefA 0.15 #2$}}}}

\coldef\bcol\Pb
\coldef\wcol\Pw
\coldef\qcol\Pq
\coldef\Qcol\PQ
\coldef\tcol\Lt
\coldef\Tcol\LT

\def\singext{\LPartition{\Lt:1}{}}
\def\upsingext{\UPartition{\Ut:1}{}}
\def\idext{
	\Partition{
	\Lt (1,0)
	\Ut (1,1)
	}}
\def\positionerext{
	\Partition{
	\Lt (1,0)
	\Ut (2,1)
	\Pline(2,0)(1,1)
	}}
\def\globcolext{
	\Partition{
	\Lt (1,0)
	\Ut (3,1)
	\Pline(2,0)(1,1)
	\Pline(3,0)(2,1)
	}}

